Mimic3D: Thriving 3D-Aware GANs via 3D-to-2D Imitation

Generating images with both photorealism and multiview 3D consistency is crucial for 3D-aware GANs, yet existing methods struggle to achieve them simultaneously. Improving the photorealism via CNN-based 2D super-resolution can break the strict 3D consistency, while keeping the 3D consistency by learning high-resolution 3D representations for direct rendering often compromises image quality. In this paper, we propose a novel learning strategy, namely 3D-to-2D imitation, which enables a 3D-aware GAN to generate high-quality images while maintaining their strict 3D consistency, by letting the images synthesized by the generator's 3D rendering branch to mimic those generated by its 2D super-resolution branch. We also introduce 3D-aware convolutions into the generator for better 3D representation learning, which further improves the image generation quality. With the above strategies, our method reaches FID scores of 5.4 and 4.3 on FFHQ and AFHQ-v2 Cats, respectively, at 512x512 resolution, largely outperforming existing 3D-aware GANs using direct 3D rendering and coming very close to the previous state-of-the-art method that leverages 2D super-resolution. Project website: https://seanchenxy.github.io/Mimic3DWeb.

==> Sections/introduction_v0.1.tex <==
\section{Introduction}
3D-aware GANs~\cite{schwarz2020graf,gu2021stylenerf,deng2022gram,chan2021efficient} have experienced rapid development in recent years. Trained with only in-the-wild 2D images, they are able to generate free-view images of virtual subjects, showing great potential for large-scale 3D content creation. The core of 3D-aware GANs is to incorporate 3D representation and differentiable renderer into their image generation process, where neural radiance field (NeRF)~\cite{mildenhall2020nerf} is the mostly adopted representation that guarantees strong 3D consistency across different viewing points.

However, incorporating NeRF into GAN training also brings high computation cost that hinders the generative models from synthesizing high-resolution images with fine details. To alleviate this problem, prior arts adopt two major strategies. The first one~\cite{niemeyer2021giraffe, gu2021stylenerf, or2022stylesdf, chan2021efficient} is to render NeRF at a lower resolution and introduces 2D super-resolution module to add high-frequency details to the rendered coarse images. 
% Rendering low-resolution NeRF largely reduces the memory cost and stablizes the training process, meanwhile the 2D super-resolution module is capable of producing fine image details at high resolution. 
A representative work among this line is EG3D~\cite{chan2021efficient}, which introduces tri-plane representation to model low-resolution NeRF and leverages StyleGAN2~\cite{karras2020analyzing}-like super-resolution module to generate high-resolution images. It sets a record for image generation quality among 3D-aware GANs and approximates that of state-of-the-art 2D GANs~\cite{karras2020analyzing, karras2021alias}. Despite the high image quality, a drawback of these line of works is a sacrifice of strict 3D consistency brought by direct 3D rendering of NeRF. The synthesized images of these methods usually suffer from geometry distortion and texture flickering issues during continuous camera change, due to the non-physical black-box synthesis process of their 2D super-resolution module.
The second group of works~\cite{deng2022gram, skorokhodov2022epigraf, schwarz2022voxgraf, zhao2022generative} thus avoid 2D super-resolution by utilizing more efficient 3D representations to allow direct rendering at a higher resolution. This brings them better 3D consistency under camera variations. Nevertheless, learning these 3D representations at high resolution is very challenging and often requires delicate training strategies~\cite{skorokhodov2022epigraf,xiang2022gram}. Some efficient representations~\cite{deng2022gram,zhao2022generative} also sacrifice the rendered quality at large viewing angles. With much effort made by the previous methods, the image generation quality among this line still falls behind those with a 2D super-resolution module, especially EG3D.

In this paper, we propose a 3D-aware GAN with direct 3D rendering that achieves state-of-the-art image generation quality. We inherit the tri-plane representation~\cite{chan2021efficient} from EG3D to efficiently model NeRF of a generated subject, and propose two key strategies to achieve high-quality image rendering without using a 2D super-resolution module, as described below:

1) \textit{3D-to-2D imitation}. Intuitively, as the images generated by EG3D are already photorealistic by leveraging a 2D super-resolution module, if we let the images produced by direct 3D rendering to mimic them, it is possible that our generator takes the advantages of both the 2D super-resolution module and the direct 3D rendering, \ie, the high image generation quality and the 3D consistency.
Based on this observation, we propose to learn a high-resolution tri-plane representation from the low-resolution one of EG3D, and let the rendered images from the high-resolution tri-planes to mimic the image content of those generated by the 2D super-resolution module. Note that the images generated by the latter sacrifice certain degrees of 3D consistency, if the rendered images try to mimic every detail of them across different views, it is likely to obtain blurry results due to detail misalignment. To avoid this problem, we only let the images produced by the two branches to be perceptually similar (\ie by LPIPS loss~\cite{zhang2018unreasonable}), and further enforce adversarial loss between the rendered images from the tri-planes and real images to maintain high-frequency details. In practice, rendering a whole image at high resolution for computing the perceptual similarity and adversarial loss can be costly. Therefore, we only render small image patches from the high-resolution tri-planes to conduct the imitative learning.

2) \textit{3D-aware tri-plane generator}. Originally, EG3D generates tri-plane features via a StyleGAN2-like generator. The generator is forced to learn 2D-unaligned features on the three orthogonal planes via 2D convolutions, which is inefficient. Inspired by a recently proposed 3D diffusion model~\cite{wang2022rodin}, we introduce 3D-aware convolution to the tri-plane generator to improve feature communications across the planes. The 3D-aware convolution considers associated features in 3D space when performing 2D convolution, which helps to produce more reasonable tri-planes. Nevertheless, directly applying 3D-aware convolution in all layers in the generator leads to unaffordable memory cost during training. As a result, we only apply them in the output layer at each resolution in the tri-plane generator. This helps us to further improve the image generation quality with only a minor increase of the total memory consumption.

With the above two strategies, our generator is able to synthesize free-view images of virtual subjects with state-of-the-art image quality. It reaches FID scores~\cite{heusel2017gans} of $3.9$ and $2.7$ on FFHQ~\cite{karras2019style} and AFHQ-v2 Cats~\cite{choi2020stargan} datasets respectively at $512\times512$ resolution, largely outperforming previous 3D-aware GANs with direct 3D rendering and even surpassing those with 2D super-resolution modules. The synthesized images are of strict 3D-consistency across multiple views, thanks to the direct volumetric rendering of the intermediate NeRF representation.

% The core intuition behind is simple: As the 2D super-resolution module can generate images with correct structures and fine details, we let the direct rendering results to mimic those generated by 2D super-resolution. In this way, we can inherit the advantages of both of them, \ie, the high quality image generation and the 3D consistency multi-view rendering. Specifically, to obtain high-quality generated images for imitation, we first train an EG3D which generates coarse tri-planes for low-resolution NeRF rendering and utilizes StyleGAN2~\cite{karras2020analyzing}-like 2D super-resolution blocks for final image synthesis. 

==> Sections/method_v0.1.tex <==
\inputfigure{fig_arch}

\section{Approach}

Sampling a vector $\mathbf z$ from the latent space, we aim to synthesize 3D-consistent high-resolution multiview images under continuous camera poses $\boldsymbol\theta$ with volume rendering method (Sec.~\ref{sec:nr}). To this end, we first propose a 3D-to-2D imitation method to train the triplane representation that has the capability for high-resolution rendering (Sec.~\ref{sec:hr}). Then, we propose a 3D aware triplane generator to improve the triplane representation with cross-plane constrained 3D information (Sec.~\ref{sec:aware3d}). The overview of our proposed method is illustrated in Fig.~\ref{fig:arch}(a).

\subsection{Volume Rendering}
\label{sec:nr}
We use the triplane representation $\mathbf P$ to model a volume. For a ray casting, we sample $N$ queries $\{\mathbf q_i\}_{i=1}^{N}$, whose features are embedded in a triplane $\mathbf P$, \ie, $\mathbf{f_q}=\mathbf{P[q]}\in\mathbb{R}^{32}$, where where $[\cdot]$ denotes grid sampling. We use an MLP-based decoder to obtain density $\sigma$ and color $\mathbf c$ as
\begin{equation}
\label{eq:decoder}
\begin{array}{l}
\mathcal{M}: \mathbf{f}\in\mathbb R^{32} \rightarrow (\mathbf c, \sigma)\in\mathbb R^4
\end{array}
\vspace{-0.1cm}
\end{equation}
We render neural fields with the volumetric method ~\cite{mildenhall2020nerf}:
% \vspace{-0.1cm}
\begin{equation}
\label{eq:render}
\begin{array}{l}
\hat{\mathbf c}=\sum_{i=1}^N T_{i}(1-\exp(-\sigma_{i} \delta_{i})) \mathbf{c}_i \\
T_i=\exp(-\sum_{j=1}^{i-1} \sigma_j \delta_j),
\end{array}
\vspace{-0.1cm}
\end{equation}
where $\delta$ is the distance between adjacent samples and $\hat{\mathbf c}$ is the RGB color of a pixel. By sampling from full view directions, we can render a fake image $\hat I$.

\subsection{Training Strategy with 3D-to-2D Imitation}
\label{sec:hr}

Prohibited by modern GPU memory, the 3D-aware GAN pipeline usually follows a small-size rendering paradigm, and a 2D super-resolution module is used to elevate image resolution. Despite high image quality, the super-resolution in image space introduces 3D inconsistency, \eg, texture flickering. 

We propose a training strategy that can achieve a high-quality 3D representation. Following the conventional 3D GAN pipeline, the training model includes a generator $G$ and a discriminator $D$, where $G=\{\mathcal E, \mathcal M, \mathcal S^{2D}\}$ with a triplane generator $\mathcal E$, decoder $\mathcal M$, and a 2D super-resolution module $\mathcal S^{2D}$. Further, we introduce a patch discriminator $D^p$ to learn from high-resolution image patches. In this manner, we limit rendering resolution up to $P=64$ to obtain an affordable memory budget. After training, we get rid of the 2D super-resolution module $\mathcal S^{2D}$ and directly render high-resolution images in the inference. 

Specifically, the strategy is divided into two stages. First, we train $\{\mathcal E, \mathcal M, \mathcal S^{2D}, D\}$ according to EG3D \cite{chan2021efficient}, and use a standard GAN loss and R1 regularization for optimization as follows,
\begin{equation}
\label{eq:gan}
\begin{aligned}
\mathcal{L}_{global}&= \mathbb{E}_{\boldsymbol{z} \sim p_z, \boldsymbol{\theta} \sim p_\theta}[f(D(G(\boldsymbol{z}, \boldsymbol{\theta})))] \\
& +\mathbb{E}_{I \sim p_{real}}[f(-D(I))+\lambda\|\nabla D(I)\|^2]
\end{aligned}
\vspace{-0.1cm}
\end{equation}
where $f(u)=\log(1+\exp{u})$ is the Softplus function, and $I$ denotes real images.

The second training stage aims to transfer the capacity of $\mathcal S^{2D}$ to $\mathcal E$. To this end, we first add an extra synthesis block to $\mathcal E$, noted as $\mathcal E^+$. $\mathcal E^+$ produces a dual triplane representation, where the pre-trained one is called coarse triplane $\mathbf P^{c}$ and the added one is named fine triplane $\mathbf P^{f}$. For a query $\mathbf q$, we sample features from the dual triplane representation as 
\begin{equation}
\label{eq:dp}
\begin{aligned}
&\mathbf{f}_{\mathbf q}^c=\mathbf P^{c}[\mathbf q] \\
&\mathbf{f}_{\mathbf q}^f=\mathbf P^{c}[\mathbf q] + \mathbf P^{f}[\mathbf q].
\end{aligned}
\vspace{-0.1cm}
\end{equation}
Then, $\{\mathcal E^{+}, \mathcal M, \mathcal S^{2D}, D, D^p\}$ is trained in an end-to-end manner with the 3D-to-2D imitation strategy. We use $\mathbf{f}_{\mathbf q}^c$ to render a full fake image $\hat I$ and leverage $\mathcal S^{2D}$ to yield the high-quality version $\hat I^{sr}$ with $F\times F$ resolution. For high-resolution training with a small rendering size $P (P<F)$, we sample queries from a random $P$ view region and use $\mathbf{f}_{\mathbf q}^f$ to render a fake image patch $\tilde I$. We crop the corresponding patch on $\hat I^{sr}$, noted as $\hat I^{sr}_{P}$, that is aligned with $\tilde I$, and let $\tilde I$ to mimic the behavior of 2D super-resolution.  However, $\hat I^{sr}_{P}$ generated by 2D super-resolution fails to perform the multi-view consistency, while $\tilde I$ from volume rendering is under a strict 3D-continuous constraint. Pixel-wise 3D-to-2D imitation could incur a sacrifice of image quality, leading to blurry results. Therefore, we leverage LPIPS loss \cite{zhang2018unreasonable} to  facilitate the imitation at the perceptual level:
\begin{equation}
\label{eq:lpips}
\begin{array}{l}
\mathcal L_{imitation}=\mathrm{LPIPS}(\tilde I, \hat I^{sr}_{P})
\end{array}
\vspace{-0.1cm}
\end{equation}
In addition, we introduce adversarial learning on image patches to further improve image quality. That is, we also crop a random $P\times P$ patch on a random real image $I$, noted as $I_{P}$, and use GAN loss to generate photo-realistic image patch:
\begin{equation}
\label{eq:patch}
\begin{aligned}
\mathcal{L}_{Patch}& = \mathbb{E}_{\boldsymbol{z} \sim p_z, \boldsymbol{\theta} \sim p_\theta}[f(D^p(G^p(\boldsymbol{z}, \boldsymbol{\theta})))] \\
& +\mathbb{E}_{I \sim p_{real}}[f(-D^p(I_{P}))+\lambda\|\nabla D(I_{P}))\|^2]
\end{aligned}
\vspace{-0.1cm}
\end{equation}
where $G^p$ performs a patch volume rendering to produce $\tilde I$.

Overall, the training objective is 
\begin{equation}
\label{eq:loss}
\mathcal L=\mathcal{L}_{global} + \mathcal{L}_{patch}+\mathcal{L}_{imitation}.
\vspace{-0.1cm}
\end{equation}


\subsection{3D Aware Triplane Generator}
\label{sec:aware3d}
The triplane representation reported by EG3D \cite{chan2021efficient} proves to be an efficient representation to model a volumetric space. However, in the 3D generative task, the generation of the triplane is less aware of 3D structure. That is, EG3D uses a StyleGAN2~\cite{karras2020analyzing} backbone to produce a feature map, which is originally designed for 2D generative tasks. Then, the feature map is divided along the channel dimension into 3 counterparts as the triplane. In this way, 
the planes for $xy$, $yz$, and $zx$ spaces are generated with individual convolutional kernels such that they are weakly aligned in 3D spaces.

To enhance the 3D structure embedded in the triplane, we develop a  3D aware generator as $\mathcal E$. As shown in Fig~\ref{fig:arch}(b), we leverage the $w$ space and modulated convolutions in StyleGAN2 to build the network. Specifically, a latent branch and a 3D-aware branch are designed to generate a 3D-structured triplane. The former is inherited from StyleGAN2 to produce a set of conventional convolutional features $\{\mathbf F_k\}$, while the latter is to generate 3D aware triplane representations $\{\mathbf P_k\}$, where $k=4,8,16,...,256$ denotes the resolution. Therefore, the latent branch models the abstract latent space while the 3D aware branch models triplane space. and they are fused with summation, $\ie$, $\mathbf P_k=\mathbf P_k+\text{conv}(\mathbf F_k)$.

The core of the 3D-aware branch is 3D-aware convolution \cite{wang2022rodin} that can fuse spatial aligned features. For example, Fig.~\ref{fig:arch}(c) illustrates the convolution process for $xy$-plane. First, a triplane representation $\mathbf P$ is split into $xy$, $yz$, $zx$ spaces, \ie, $\mathbf P_{xy},\mathbf P_{yz},\mathbf P_{zx}$. To align $\mathbf P_{yz}$ and $\mathbf P_{zx}$ spaces towards $\mathbf P_{xy}$, we perform global pooling along $z$ axis to obtain $z$-squeezed feature vectors. Then, the vector is repeated along the original $z$ dimension to obtain the original spatial size, denoted as $\mathbf P_{yr},\mathbf P_{rx}$. In this manner $\mathbf P_{yr},\mathbf P_{rx}$ is 3D-spatially aligned with $\mathbf P_{xy}$, and they are concatenated to evolve $\mathbf P^{xy}$, $\mathbf P_{2k,xy}=\text{conv}([\mathbf P_{k,xy},\mathbf P_{k,yr},\mathbf P_{k,rx}])$. Similarly, $\mathbf P_{yz}$ and $\mathbf P_{zx}$ can be processed with 3D aware convolution.

Our two-stream design has two-fold advantages over that in \cite{wang2022rodin} in terms of generative tasks. First, three planes are usually with unequal importance, \eg, $xy$ plane usually dominates the model performance in FFHQ data distribution. Therefore, instead of splitting a latent feature into three counterparts with the same channel size like \cite{wang2022rodin}, our latent branch can adaptively assign computation budgets for three inequivalent spaces. Second, as shown in Fig.~\ref{fig:arch}(c), 3D-aware convolution is memory unfriendly by introducing multiple auxiliary tensors. Our 3D-aware operation is conducted on the triplane, which is much more memory-efficient than the latent feature. 



==> Tables/tab_mem.tex <==
\begin{table}[t]
\small
\renewcommand{\arraystretch}{1.2}
% \setlength\tabcolsep{2pt}
\centering
\begin{tabular}{c | c c c | c}
\hline
Label & $\mathcal{L}_{imitation}$ & $\mathcal S^{3D}$ & $\mathcal{L}_{adv}^{3D}$ & FID (3D branch) \\ 
\hline 
(A) &             &              &  & 30.6 \\
(B) & \checkmark  &              &  & 29.9 \\
(C) & \checkmark  & \checkmark   &  & 9.29 \\
(D) &             & \checkmark   & \checkmark & 22.8 \\
(E) & \checkmark  & \checkmark   & \checkmark &  \textbf{5.14}\\
\hline
\end{tabular}
\caption{Ablation study on 3D-to-2D imitation strategy.}
\label{tab:sr}
\vspace{-0.1cm}
\end{table}


==> Tables/tab_plane.tex <==
\begin{table}[t]
\small
%\renewcommand{\arraystretch}{1.}
% \setlength\tabcolsep{2pt}
\centering
\begin{tabular}{c | c c c }
\hline
Method & $xy$ & $yz$ & $zx$ \\
\hline 
EG3D \cite{chan2021efficient} & 2.11 & 1.96 & 1.09  \\
Ours & 3.31 & 2.51 & 2.34  \\
\hline
\end{tabular}
\caption{Information entropy of different triplane representations.}
\label{tab:entropy}
% \vspace{-0.1cm}
\end{table}
